Improving Gibbs Sampler Scan Quality with DoGS

The pairwise influence matrix of Dobrushin has long been used as an analytical tool to bound the rate of convergence of Gibbs sampling. In this work, we use Dobrushin influence as the basis of a practical tool to certify and efficiently improve the quality of a discrete Gibbs sampler. Our Dobrushin-optimized Gibbs samplers (DoGS) offer customized variable selection orders for a given sampling budget and variable subset of interest, explicit bounds on total variation distance to stationarity, and certifiable improvements over the standard systematic and uniform random scan Gibbs samplers. In our experiments with joint image segmentation and object recognition, Markov chain Monte Carlo maximum likelihood estimation, and Ising model inference, DoGS consistently deliver higher-quality inferences with significantly smaller sampling budgets than standard Gibbs samplers.

==> expideas.tex <==


\section{Ideas for more experiments}


	\bitemize
		\item Evaluating scan quality
		\bitemize
			\item Show that scan quality can beused to select between random scan and systematic scan 
			\item Perhaps in two different cases: one in which random scan is much better in practice and one in which systematic scan is much better
			\item Relevant sources for models / inference tasks?
			\bitemize
				\item Roberts Rosenthal - Surprising Convergence Properties of Some Simple Gibbs Samplers under Various Scans : \url{http://probability.ca/jeff/ftpdir/55570-192935-1-SM.pdf}
			\eitemize
		\eitemize
		\item Improving total variation
		\bitemize
			\item for simulated datasets,  show that our full total variation bound is much better than systematic / random scan and show that the sample points obtained are in fact better w.r.t. full total variation
			\item for a real dataset, show that our full total variation bound is much better than systematic / random scan and show that the sample points obtained are in fact better based on some metric meaningful in that task (use either an MRF experiment or an LDA experiment for this one)
			\item Methods to compare
			\bitemize
				\item Method of \cite{levine2006optimizing}?
				\item (Uniform) random update
				\item Systematic scan
				\item Minimum spectral norm q?
				\item Single q, optimized with gradient descent
				\bitemize
					\item Initialized at (uniform) random update
					\item Perhaps we should check whether a random initialization leads to significantly different results
				\eitemize
				\item Multi-q coordinate descent
				\bitemize
					\item Initialized with (uniform) random update
					\item Initialized with systematic scan
					\item Initialized with minimum spectral norm q?
				\eitemize
			\eitemize
		\eitemize
		\item Improving marginal total variation
		\bitemize 
			\item for simulated datasets and each finite number of steps T, show that we obtain a better bound than standard Gibbs sampling and even than q optimized for full total variation, and show that the sample points obtained are in fact better w.r.t. marginal total variation
			\item for a real dataset inference task (in which we would only care about particular marginals) and each finite number of steps T, show that we obtain a better bound than standard Gibbs sampling and even than scan optimized for full total variation, and show that the sample points obtained are in fact better based on some metric meaningful in that task (use either an MRF experiment or an LDA experiment for this one, whichever wasn't used before)
		\eitemize
		\item \notate{Sources of inspiration for experiments}
		\bitemize
			\item Projecting Markov Random Field Parameters for Fast Mixing \url{https://papers.nips.cc/paper/5315-projecting-markov-random-field-parameters-for-fast-mixing.pdf}
			\bitemize
				\item Describes how to bound influence matrix in any pairwise Markov random field (we should note this in our paper too!)
				\item Berkeley binary image denoising experiment
				\bitemize
					\item \notate{Promising for improving full total variation}: use the same data, noise, and denoising model; just set pairwise strength parameter to be in the Dobrushin regime 
					\item \notate{Is this also an interesting experimental setup for marginal TV?  What marginals would we be interested in?  What about the Ioannis's enhance motivation: in some cases, we may be principally interested in denoising a small region of the image (e.g., the center m x m pixel square?}
				\eitemize
				\item Synthetic experiment recovering marginals of Ising models
			\eitemize
			\item Optimizing random scan Gibbs samplers \url{http://www.sciencedirect.com/science/article/pii/S0047259X06000613}
			\bitemize
				\item Experiments on Bayesian mixture models 
				\item Experiments on Dirichlet process mixture models
			\eitemize
			\item Other papers on fast Gibbs sampling?
			\item \url{http://vcla.stat.ucla.edu/old/MCMC/MCMC_tutorial/Lect2_Basic_MCMC.pdf}
			\bitemize
				\item Mentions edge classification as an application of Gibbs
			\eitemize
			\item Verbeek Triggs - Region Classification with Markov Field Aspect Models - CVPR07.pdf
			\bitemize
				\item Train the Markov aspect model, fix the learned parameters (like the thetas and betas), and carry out topic inference using Gibbs sampling; in this case, the only influence between variables is due to the Markov random field potentials; the Potts potentials in the MRF must be set to obey Dobrushin's condition
				\item Key Problem: all documents (images) are independent when parameters are fixed, so really only sampling for a single document at a time; in addition, if we ignore boundary effects, then the influence is identical between all pairs of variables (so you might think that uniform / systematic scan is optimal for full total variation); this seemingly makes this application unsuitable both for demoing improved marginal total variation and improved full total variation; \notate{if edge effects are significant, so that uniform sampling is far from optimal, then could be used for improved full total variation}
			\eitemize
			\item COUPLING HIDDEN MARKOV MODELS FOR THE DISCOVERY
OF CIS-REGULATORY MODULES IN MULTIPLE SPECIES \url{http://arxiv.org/pdf/0708.4318.pdf}
			\bitemize
				\item Awesome application, but may take a while to parse the model and learn if its Dobrushin-friendly
			\eitemize	
			\item Markov Random Field Modeling in Image Analysis \url{http://read.pudn.com/downloads139/ebook/596264/Markov_Random_Field_modeling_in_Image_Analysis_by_Stan_Z.Li.pdf}
			\bitemize
				\item Describes a variety of applications of MRF modeling in image analysis
				\item Example: generating textures with Gibbs sampling \notate{could be suitable for improved full total variation}
			\eitemize
			\item Explores Semi-restricted boltzmann machines for handwritten digit modeling: \url{http://www.cs.toronto.edu/~rsalakhu/papers/bm.pdf}
			\item Describes collapsed Gibbs sampler for Gaussian mixture model \url{http://www.kamperh.com/notes/kamper_bayesgmm13.pdf}
			\bitemize
				\item Will this have the same problem as LDA (need for strong prior parameters)?
			\eitemize
			\item Rapidly Mixing Gibbs Sampling for a Class of Factor Graphs Using Hierarchy Width \url{https://papers.nips.cc/paper/5757-rapidly-mixing-gibbs-sampling-for-a-class-of-factor-graphs-using-hierarchy-width.pdf}
			\bitemize
				\item To validate this, we constructed a hierarchical template for the Paleontology application used by Shanan et al. [17].
				\item we chose a subgraph of a KBP system used by Shin et al. [20] that can be grounded by a hierarchical template and chose a setting of the weight such that the true marginal was 0.5 for all variables. We then ran Gibbs sampling on this subgraph and report the average error of the marginal estimation in Figure 5(b).
			\eitemize
			\item Maximum Likelihood Learning With ArbitraryTreewidth via Fast-Mixing Parameter Sets \url{http://papers.nips.cc/paper/5907-maximum-likelihood-learning-with-arbitrary-treewidth-via-fast-mixing-parameter-sets.pdf}
			\bitemize
				\item \notate{Can conduct an experiment on improving MCMC-MLE!}
				\item Use the exact Ising model experiment from this paper and compare the convergence of parameter values using uniformly random Gibbs sampling vs. using our optimized scans
				\item One option is to use the number of sampling steps used in this paper for both chains (standard Gibbs vs. optimized Gibbs); I believe that number of sampling steps was chosen to achieve a certain bound on total variation $\epsilon_\theta$ and plot parameter estimate vs. number of parameter updates
				\item A second option is to use the same value of $\epsilon_\theta$ for both chains and use our procedure to determine the smallest number of sample points needed to get a guarantee of $\epsilon_\theta$ with an optimized scan; presumably then our optimized scan chain would use fewer sample points, so we could plot parameter estimates vs. number of sample points used
			\eitemize
		\eitemize
	\eitemize
